HyDe: The First Open-Source, Python-Based, GPU-Accelerated Hyperspectral Denoising Package

As with any physical instrument, hyperspectral cameras induce different kinds of noise in the acquired data. Therefore, Hyperspectral denoising is a crucial step for analyzing hyperspectral images (HSIs). Conventional computational methods rarely use GPUs to improve efficiency and are not fully open-source. Alternatively, deep learning-based methods are often open-source and use GPUs, but their training and utilization for real-world applications remain non-trivial for many researchers. Consequently, we propose HyDe: the first open-source, GPU-accelerated Python-based, hyperspectral image denoising toolbox, which aims to provide a large set of methods with an easy-to-use environment. HyDe includes a variety of methods ranging from low-rank wavelet-based methods to deep neural network (DNN) models. HyDe's interface dramatically improves the interoperability of these methods and the performance of the underlying functions. In fact, these methods maintain similar HSI denoising performance to their original implementations while consuming nearly ten times less energy. Furthermore, we present a method for training DNNs for denoising HSIs which are not spatially related to the training dataset, i.e., training on ground-level HSIs for denoising HSIs with other perspectives including airborne, drone-borne, and space-borne. To utilize the trained DNNs, we show a sliding window method to effectively denoise HSIs which would otherwise require more than 40 GB. The package can be found at: \url{https://github.com/Helmholtz-AI-Energy/HyDe}.

==> more_detailed_methods.tex <==
First Order Spectral Roughness Penalty Denoising (FORPDN)~\cite{forpdn} is a full-rank, wavelet-based model which solves a minimization problem involving the noise covariance matrix, a $(p-1)\times p$ difference matrix, and the multiresolution property of wavelet decomposition.
Certain parameter values of the minimization problem are determined automatically via the Stein's unbiased risk estimate (SURE)~\cite{SURE}. 
This method is primarily for removing Gaussian noise.

% \subsubsection{FastHyDe, FastHyIn, and L1HyMixDe}
% \label{sec:fasthyde}
Fast Hyperspectral Denoising (FastHyDe)~\cite{fasthyde} is a low-rank method based on sparse representations.
It uses the HySime~\cite{HySime} and BM3D~\cite{bm3d} methods.
The method of HySime is easily parallelized and included in HyDe.
BM3D is a closed source package and is dependent on NumPy. 
This forces BM3D to operate on CPU exclusively.
FastHyDe is primarily for removing Gaussian and/or Poissonian noise.

The Fast Hyperspectral Inpainting method (FastHyIn)~\cite{fasthyde} is very similar to FastHyDe.
The only difference is the inclusion of an inpainting mask which is added to the noisy image before the noise is estimated. 
This allows FastHyIn to remove Gaussian and Sparse noise while also filling in missing data.

The Hyperspectral Mixed Noise Removal By $\ell_1$-Norm-Based Subspace Representation (L1HyMixDe)~\cite{l1hymixde} method is built on top of FastHyIn.
Its stated objective is to exploit a compact and sparse representation of the input's rank and self-similarity characteristics.  
This method can remove mixtures of Gaussian noise and sparse noise.

% \subsubsection{HyRes and HyMiNoR}
% \label{sec:hyres}
Automatic Hyperspectral Restoration (HyRes)~\cite{hyres} is a low-rank, wavelet-based method which uses SVD on a 2D projection of the HSI, wavelet decomposition, and Hyperspectral SURE \cite{HySURE} to estimate the noise.
These methods form a parameter-free, high-level method primarily used for removing additive Gaussian noise.

Hyperspectral Mixed Gaussian and Sparse Noise Reduction (HyMiNoR)~\cite{hyminor} is a low-rank, wavelet-based method build on top of HyRes.
First, the Gaussian noise is removed by HyRes, then, the remaining noise (of differing types) is removed by solving an $\ell_1$-$\ell_1$ optimization problem using a modified split-Bregman technique.
This method is intended for removing mixtures of Gaussian noise and sparse noise.

% \subsubsection{WSRRR}
% \label{sec:wsrrr}
Wavelet-Based Sparse Reduced-Rank Regression (WSRRR)~\cite{wsrrr} is a low-rank, wavelet-based method which minimizes a sparse regularization problem with an orthogonality constraint. 
It uses a cyclic descent minimization algorithm, with tuning parameters determined by SURE.
This method is intended for removing Gaussian noise and extracting features.

% \subsubsection{OTVCA}
% \label{sec:otvca}
Orthogonal Total Variation Component Analysis (OTVCA) \cite{otvca} is a low-rank, feature extraction method.
Features are extracted using a total variation penalized optimization problem. 
This method uses a SciPy~\cite{scipy} implementation of split-Bregman optimization to perform the total-variation denoising. 
This method is intended for removing Gaussian noise and extracting features.

Due to dependences, OTVCA, FastHyDe, FastHyIn, and L1HyMixDe do not effectively utilize GPUs.
